Procedural Generation of Complex Roundabouts for Autonomous Vehicle Testing

High-definition roads are an essential component of realistic driving scenario simulation for autonomous vehicle testing. Roundabouts are one of the key road segments that have not been thoroughly investigated. Based on the geometric constraints of the nearby road structure, this work presents a novel method for procedurally building roundabouts. The suggested method can result in roundabout lanes that are not perfectly circular and resemble real-world roundabouts by allowing approaching roadways to be connected to a roundabout at any angle. One can easily incorporate the roundabout in their HD road generation process or use the standalone roundabouts in scenario-based testing of autonomous driving.

==> contents/acknowledgement.tex <==
\section*{Acknowledgment}

==> contents/conclusion.tex <==
\section{CONCLUSIONS}
In this paper, we have presented detailed approach of how JunctionArt, our generator, can generate Classic and Turbo roundabouts. 

==> contents/future_work.tex <==
\section{Future Work}
% 1. variation in turbo-roundabouts
While variations in both roundabouts were thoroughly presented in this work, there are many variation in turbo roundabouts that still needs to be addressed such as shape, number of spikes etc. Many roundabouts have slip roads that are adjacent to or even sometimes partially overlapping with the roundabout area. We left such designs for future scope.

Improvement on distortion algorithm - learning real-world distortion dis tribution, more algorithms that can generate different shapes (we saw some mango-shaped roundabouts in real-world) @@@ example.


Besides, a further study into the randomization algorithm can improve the stability and effectiveness of the outputs. To achieve this, neural networks may be proven effective.
% 2. improvement on randomization algorithm to control output shapes.

==> contents/methods.tex <==
\section{METHODS FOR ROUNDABOUT GENERATION}
% define terminology
In this section, we present our approaches in creating two types of roundabouts: (a) classical roundabout, (b) turbo roundabout. 
% @@@ define both roundabouts and show two pictures. 
\input{tables-figures/roundabout_classification.tex}

% our sample roundabouts and its structures, definitions/terms.
A roundabout is a set of roads of two types: circular roads and incident roads. Vehicles approach and leave the roundabout through one of the incident roads. Circular roads create the loop inside the roundabout and connect the incident roads. Furthermore, we define the \textit{incident road definition} as a four-value tuple(position, heading, noOfLeftLanes, noOfRightLanes). Each incident road definition corresponds to the incident point where an incident road is connected to the roundabout area. Given a set of incident road definitions, a roundabout is generated in three phases. In the first phase, we find a circle using the incident points. In the second phase, we create the circular roads. In the third phase, we create incident roads and connect them to circular roads using connection roads.

In our work, we refer classic roundabouts as the standard multi-lane roundabouts. Turbo roundabouts@@@cite refer to the roundabouts with enhanced design for disallowing lane changing, which minimizes conflict points .


\input{methods/classic.tex}
\input{methods/turbo.tex}




==> contents/references.tex <==
\section*{References}


==> methods/algorithm.tex <==
\algnewcommand\algorithmicforeach{\textbf{for each}}
\algdef{S}[FOR]{ForEach}[1]{\algorithmicforeach\ #1\ \algorithmicdo}

\begin{algorithm}
\caption{Straight Road Generation Using Road Definition}
\label{alg:road_generation}
\begin{algorithmic}[1]
    \Procedure{generateOffsets}{$startingPoint, center$}
    \State $offsets\gets[]$
    \ForEach {$startingPoint \in startingPoints$} 
        \State $heading \gets startingPoint_{heading}$
        \If{$heading \ge \pi$}
            \State $heading \gets heading - 2\pi$
        \ElsIf{$heading < -\pi$}
            \State $heading \gets heading + 2\pi$
        \EndIf
        \State $radius \gets gradient(center, startPoint)$
        \State $heading_{radius} \gets tan^{-1}(radius)$ 
        \State $offset \gets heading_{radius} - heading$
        \State \textbf{Push} $offset$ to $offsets$
    \EndFor
    \Return $offsets$
    \EndProcedure
    \State
    \Procedure{CreateStraightRoad}{startPoint, center, radius, nLane}
        \State $d \gets Distance(startPoint, center)$ 
        \If{$d > 1.5*radius \And |offset_{startPoint}| < 1$}
            \State $ k \gets (1 - |offset_{startPoint}|)$
            \State $length_{road} \gets k(d - 1.5*radius)$
        \Else \State $length_{road} = 0$
        \EndIf
        \State \textbf{Create} straight road with $length_{road}$ length and $nLane$ lanes
    \EndProcedure
\end{algorithmic}
\end{algorithm}

==> tables-figures/peanutroundabout.tex <==
\begin{figure}[bt!]
    \centering
    \framebox{\includegraphics[width=.9\linewidth]{images/peanut.png}}
    \caption{Peanut shaped roundabout from Sunbury, Ohio 43074, USA. Map data \textcopyright 2023 Google}
    \label{fig:peanutroundabout}
\end{figure}

==> templates/1-figure.tex <==
\begin{figure}[bt!]

    \centering
    \framebox{\includegraphics[width=.9\linewidth]{images/crosswalk-area-1.PNG}}
    \caption{(a) K-shaped with one road having median restricted lanes (right bottom), (b) long-connections, (c) single outgoing lane road in a 3-way intersection.}
    \label{fig:2-sub-figure}
\end{figure}

==> templates/2-sub-figure.tex <==
\begin{figure}[bt!]
    \begin{subfigure}[b]{.5\linewidth}
      \centering
      \framebox{\includegraphics[width=.9\linewidth]{images/crosswalk-area-1.PNG}}
      \caption{}
      \label{fig:4-way-k}
    \end{subfigure}%%
    \begin{subfigure}[b]{.5\linewidth}
      \centering
      \framebox{\includegraphics[width=.9\linewidth]{images/crosswalk-area-midblock.PNG}}
      \caption{}
    \end{subfigure}
    \caption{(a) K-shaped with one road having median restricted lanes (right bottom), (b) long-connections, (c) single outgoing lane road in a 3-way intersection.}
    \label{fig:2-sub-figure}
\end{figure}

==> templates/table.tex <==
Place figures and tables at the top and 
bottom of columns. Avoid placing them in the middle of columns. Large 
figures and tables may span across both columns. Figure captions should be 
below the figures; table heads should appear above the tables. Insert 
figures and tables after they are cited in the text. Use the abbreviation 
``Fig.~\ref{fig}'', even at the beginning of a sentence.

\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table}

\begin{figure}[htbp]
\centerline{\includegraphics{fig1.png}}
\caption{Example of a figure caption.}
\label{fig}
\end{figure}

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words 
rather than symbols or abbreviations when writing Figure axis labels to 
avoid confusing the reader. As an example, write the quantity 
``Magnetization'', or ``Magnetization, M'', not just ``M''. If including 
units in the label, present them within parentheses. Do not label axes only 
with units. In the example, write ``Magnetization (A/m)'' or ``Magnetization 
\{A[m(1)]\}'', not just ``A/m''. Do not label axes with a ratio of 
quantities and units. For example, write ``Temperature (K)'', not 
``Temperature/K''.

